INTERLEAVE: A Faster Symbolic Algorithm for Maximal End Component Decomposition

This paper presents a novel symbolic algorithm for the Maximal End Component (MEC) decomposition of a Markov Decision Process (MDP). The key idea behind our algorithm INTERLEAVE is to interleave the computation of Strongly Connected Components (SCCs) with eager elimination of redundant state-action pairs, rather than performing these computations sequentially as done by existing state-of-the-art algorithms. Even though our approach has the same complexity as prior works, an empirical evaluation of INTERLEAVE on the standardized Quantitative Verification Benchmark Set demonstrates that it solves 19 more benchmarks (out of 379) than the closest previous algorithm. On the 149 benchmarks that prior approaches can solve, we demonstrate a 3.81x average speedup in runtime.

==> packages.tex <==
\RequirePackage{amsmath}
\usepackage{algorithm}
\usepackage{amssymb,mathtools}
\usepackage[noEnd=true,indLines=true]{algpseudocodex}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
% \usepackage{xpatch}
% \makeatletter
% \xpatchcmd{\algorithmic}{\itemsep\z@}{\itemsep=2ex plus1pt}{}{}
% \makeatother

%
\usepackage[T1]{fontenc}
\usepackage{graphicx}
\graphicspath{{images/}}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=Maroon,
    filecolor=Maroon,      
    citecolor=Blue,
    urlcolor=Blue,
    pdftitle={An Empirically Faster Symbolic Algorithm for MEC Decompositon of MDPs},
    pdfpagemode=FullScreen,
    pdfcreator={LaTeX via pandoc},
    }
\urlstyle{same} % disable monospaced font for URLs

% Used for displaying a sample figure. If possible, figure files should
% be included in EPS format.
%
% If you use the hyperref package, please uncomment the following two lines
% to display URLs in blue roman font according to Springer's eBook style:
\usepackage{color}
\renewcommand\UrlFont{\color{blue}\rmfamily}
\urlstyle{rm}
%

\usepackage{booktabs}
\usepackage[caption=false]{subfig}
% \usepackage{subcaption}
\usepackage{enumitem}
\usepackage{setspace,float}

\usepackage{svg}
\usepackage{tikz}
\usetikzlibrary{automata, positioning, arrows}
\tikzset{
->, % makes the edges directed
>=stealth, % makes the arrow heads bold
node distance=3cm, % specifies the minimum distance between two nodes. Change if necessary.
every state/.style={thick}, % sets the properties for each ’state’ node
every scc/.style={thick, fill=green!10},
every rest/.style={thick, fill=yellow!10},
initial text=$ $, % sets the text that appears on the start arrow
}
\usepackage{longtable}

\usepackage{comment}

\usepackage{orcidlink}
